Cooperative Assistance in Robotic Surgery through Multi-Agent Reinforcement Learning

Cognitive cooperative assistance in robot-assisted surgery holds the potential to increase quality of care in minimally invasive interventions. Automation of surgical tasks promises to reduce the mental exertion and fatigue of surgeons. In this work, multi-agent reinforcement learning is demonstrated to be robust to the distribution shift introduced by pairing a learned policy with a human team member. Multi-agent policies are trained directly from images in simulation to control multiple instruments in a sub task of the minimally invasive removal of the gallbladder. These agents are evaluated individually and in cooperation with humans to demonstrate their suitability as autonomous assistants. Compared to human teams, the hybrid teams with artificial agents perform better considering completion time (44.4% to 71.2% shorter) as well as number of collisions (44.7% to 98.0% fewer). Path lengths, however, increase under control of an artificial agent (11.4% to 33.5% longer). A multi-agent formulation of the learning problem was favored over a single-agent formulation on this surgical sub task, due to the sequential learning of the two instruments. This approach may be extended to other tasks that are difficult to formulate within the standard reinforcement learning framework. Multi-agent reinforcement learning may shift the paradigm of cognitive robotic surgery towards seamless cooperation between surgeons and assistive technologies.

==> IROS2021 - ArXiv - Cooperative Assistance/network.tex <==

\begin{figure}[tb]
  \centering
  %\hspace*{-0.75cm}
  \vspace{1.5mm}
  \begin{tikzpicture}
    \node[rotate=90] (img) at (0,0) {\small$z_t$};

    \node[conv,rotate=90,minimum width=3.3cm] (conv1) at (0.8,0) {\small$\text{conv}_{4k, 1s, 32c}$ + $\ReLU$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv2) at (1.6,0) {\small$\text{conv}_{4k, 1s, 64c}$ + $\ReLU$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv3) at (2.4,0) {\small$\text{conv}_{4k, 1s, 128c}$ + $\ReLU$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv4) at (3.2,0) {\small$\text{conv}_{4k, 1s, 256c}$ + $\ReLU$};
    \node[conv,rotate=90,minimum width=3.3cm] (conv5) at (4,0) {\small$\text{conv}_{4k, 1s, 512c}$ + $\ReLU$};
    \node[fc  ,rotate=90,minimum width=3.3cm] (fc1) at (4.8,0) {\small$\text{fc}_{1024}$};
    
    \node[rotate=90] (action) at (0,1) {\small $a_{i, t-1}$};
    
    \node[lstm,rotate=90,minimum width=3.3cm] (lstm) at (5.6,0) {\small$\text{LSTM}_{512}$};
    \node[fc  ,rotate=90,minimum width=3.3cm] (fc2) at (6.4,0) {\small$\text{fc}_{1024}$ + $\ReLU$};
    \node[fc  ,rotate=90,minimum width=3.3cm] (fc3) at (7.2,0) {\small$\text{fc}_{10}$};

    \node[rotate=90] (act) at (8,1) {\small$\pi_{i, t}$};
    \node[rotate=90] (val) at (8,-1) {\small$V_{i, t}$};


    \draw[->] (img) -- (conv1);
    \draw[->] (conv1) -- (conv2);
    \draw[->] (conv2) -- (conv3);

    \draw[->] (conv3) -- (conv4);
    \draw[->] (conv4) -- (conv5);

    \draw[->] (conv5) -- (fc1);
    \draw[->] (fc1) -- (lstm);

    \draw[->] (lstm) -- (fc2);
    \draw[->] (fc2) -- (fc3);

    \draw[->] (fc3) -- (act);
    \draw[->] (fc3) -- (val);
    
    \draw[->] (action.east) -- node {} (0, 2) -| (lstm.east);

  \end{tikzpicture}
  \caption{Illustration of the artificial agents' neural networks. Convolutional layers (kernel size $k$, stride $s$, channel $c$), followed by a combination of fully connected and LSTM layers. Outputs are logits ($\pi_{i, t}$) and value ($V_{i, t}$).}
  \label{fig:network}
  \vspace{-0.6cm}
\end{figure}


==> IROS2021 - ArXiv - Cooperative Assistance/plots/learning_curve.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.266666666666667,0.466666666666667,0.666666666666667}
\definecolor{color1}{rgb}{0.933333333333333,0.4,0.466666666666667}
\definecolor{color2}{rgb}{0.133333333333333,0.533333333333333,0.2}
\definecolor{color3}{rgb}{0.8,0.733333333333333,0.266666666666667}

\begin{axis}[
x grid style={white!69.0196078431373!black},
xlabel={\scriptsize Total Environment Steps},
xmin=-288288, xmax=7152288,
xtick pos=both,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\scriptsize Discounted Return},
ymin=-22.1813958573089, ymax=-7.27974484059465,
ytick pos=left,
ytick style={color=black}
]
\addplot [very thick, color0]
table {%
49920 -21.5040480838219
74880 -21.1827974647543
99840 -20.7382724465402
124800 -20.4181807455722
149760 -20.1672456540431
174720 -20.0306862873427
199680 -20.108840957863
224640 -20.0768693775711
249600 -20.0378520216418
274560 -20.0484475850687
324480 -19.8513096398831
374400 -19.702423021939
424320 -19.617712030216
474240 -19.5958992299732
524160 -19.5588585185347
574080 -19.5899820385266
624000 -19.4616895139411
673920 -19.3399181157626
723840 -19.2805551285742
773760 -19.1953316922821
823680 -19.1330114576469
873600 -19.1003669646225
923520 -19.0770256191707
973440 -18.9917650777353
1023360 -18.9892890571493
1073280 -18.9419460988782
1123200 -18.8416428681302
1173120 -18.7880762867179
1223040 -18.6650964808592
1272960 -18.3926056123042
1322880 -17.969604018927
1372800 -17.4307253986179
1422720 -16.9022332596665
1472640 -16.4140599940098
1522560 -15.9027247871292
1572480 -15.3560557761683
1622400 -14.8832678631575
1672320 -14.4070487135294
1722240 -13.9299480521507
1772160 -13.5643457671856
1822080 -13.3919921497161
1872000 -13.491008567069
1921920 -13.6495731080686
1971840 -13.6608632360486
2021760 -13.6251105166927
2071680 -13.5907730054541
2121600 -13.5631835746639
2171520 -13.5565636511123
2221440 -13.5604444871481
2271360 -13.5584916698884
2321280 -13.567112531402
2371200 -13.4477978259416
2421120 -13.2271443184031
2471040 -13.0863694027688
2520960 -13.0067422858907
2570880 -12.9995341474053
2620800 -13.1005547885826
2670720 -13.2478727952339
2720640 -13.4528035787561
2770560 -13.6331957449306
2820480 -13.5828257540864
2870400 -13.3001354649258
2920320 -13.0451509928973
2970240 -12.848182217605
3020160 -12.5773408160109
3070080 -12.2527934928604
3120000 -11.8524058616213
3169920 -11.4460235276974
3219840 -10.9103904471533
3269760 -10.3758936058991
3319680 -10.1493774685482
3369600 -10.0611940761428
3419520 -10.2197463160194
3469440 -10.1352382335704
3519360 -10.1267905929482
3569280 -10.0011823692447
3619200 -9.88124232622069
3669120 -9.64674547547582
3719040 -9.5245430163311
3768960 -9.43407828971426
3818880 -9.27540347530714
3868800 -9.10150903485422
3918720 -8.71699690554348
3968640 -8.58279913649857
4018560 -8.51728603798155
4068480 -8.48575773869541
4118400 -8.39866930883652
4168320 -8.39731709804498
4218240 -8.36287584317581
4268160 -8.35503501809728
4318080 -8.2807509426549
4368000 -8.30833266943386
4417920 -8.32450831899301
4467840 -8.33281282756494
4517760 -8.23518912028296
4567680 -8.19406078473346
4617600 -8.19622377358428
4667520 -8.17646914452722
4717440 -8.15214283190572
4767360 -8.12502481377371
4817280 -8.14960576665908
4867200 -8.14080271033512
4917120 -8.16441442520513
4967040 -8.14264039263577
5016960 -8.14074911589156
5066880 -8.13263549562361
5116800 -8.12330619505144
5166720 -8.11831066092713
5216640 -8.11549596177326
5266560 -8.09403924244443
5316480 -8.08351237392855
5366400 -8.05991360155514
5416320 -8.00142823627823
5466240 -8.01630599061512
5516160 -8.01839797688231
5566080 -8.01551814234745
5616000 -7.99695626918515
5665920 -8.01534030314152
5715840 -8.00138148613027
5765760 -7.99625540525388
5815680 -7.98587233202064
5865600 -8.01583181973664
5915520 -8.04199977527534
5965440 -8.04095356090127
6015360 -8.05091459449297
6065280 -8.0429501848792
6115200 -8.05614699202149
6165120 -8.0502487393353
6215040 -8.05222055260378
6264960 -8.07653399641677
6314880 -8.07916527726033
6364800 -8.04066320719996
6414720 -8.0273415804971
6464640 -8.05116276585494
6514560 -8.03536637890315
6564480 -8.03292787783407
6614400 -8.00431567053931
6664320 -7.97955364769339
6714240 -7.99436547182909
6764160 -7.97718630405352
6814080 -7.95709261408166
};
\label{plot1}
\end{axis}

\begin{axis}[
axis y line=right,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.91,0.5)}, anchor=east, draw=none},
x grid style={white!69.0196078431373!black},
xmin=-288288, xmax=7152288,
xtick pos=both,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Outcome (\%)},
ymin=0, ymax=105,
ytick pos=right,
ytick style={color=black},
yticklabel style={anchor=west}
]
\addplot [very thick, color1]
table {%
49920 0
74880 18.5
99840 43.6666666666667
124800 50.5
149760 46.4
174720 43.8333333333333
199680 48.7142857142857
224640 54.875
249600 59
274560 61
324480 70.2
374400 76.5
424320 77.1
474240 80
524160 87
574080 93.9
624000 96.1
673920 96.3
723840 97
773760 98.9
823680 99.7
873600 97.5
923520 91
973440 82.7
1023360 74.5
1073280 69.5
1123200 68
1173120 67.7
1223040 65.3
1272960 59
1322880 49.9
1372800 42.1
1422720 38.6
1472640 36.9
1522560 35.1
1572480 30.1
1622400 21.6
1672320 12
1722240 4.7
1772160 1.3
1822080 0.4
1872000 0.4
1921920 0.4
1971840 0.4
2021760 0.4
2071680 0.5
2121600 0.6
2171520 0.5
2221440 0.3
2271360 0.2
2321280 0.2
2371200 0.2
2421120 0.2
2471040 0.2
2520960 0.2
2570880 0.1
2620800 0
2670720 0.1
2720640 0.2
2770560 0.2
2820480 0.3
2870400 0.4
2920320 0.4
2970240 0.4
3020160 0.5
3070080 0.6
3120000 0.8
3169920 0.8
3219840 0.7
3269760 0.8
3319680 0.7
3369600 0.6
3419520 0.6
3469440 0.6
3519360 0.5
3569280 0.4
3619200 0.2
3669120 0.1
3719040 0.1
3768960 0
3818880 0
3868800 0
3918720 0
3968640 0
4018560 0
4068480 0
4118400 0
4168320 0
4218240 0
4268160 0
4318080 0
4368000 0
4417920 0
4467840 0
4517760 0
4567680 0
4617600 0
4667520 0.1
4717440 0.1
4767360 0.1
4817280 0.1
4867200 0.1
4917120 0.1
4967040 0.1
5016960 0.1
5066880 0.1
5116800 0.1
5166720 0
5216640 0
5266560 0
5316480 0
5366400 0
5416320 0
5466240 0
5516160 0
5566080 0
5616000 0
5665920 0
5715840 0
5765760 0
5815680 0
5865600 0
5915520 0
5965440 0
6015360 0
6065280 0
6115200 0
6165120 0
6215040 0.1
6264960 0.1
6314880 0.1
6364800 0.1
6414720 0.1
6464640 0.1
6514560 0.2
6564480 0.2
6614400 0.2
6664320 0.2
6714240 0.1
6764160 0.1
6814080 0.1
};
\addlegendentry{\scriptsize{Lost Grasp}}
\addplot [very thick, color2]
table {%
49920 100
74880 81.5
99840 56.3333333333333
124800 49.5
149760 53.6
174720 56.1666666666667
199680 51.2857142857143
224640 45.125
249600 41
274560 39
324480 29.8
374400 23.5
424320 22.9
474240 20
524160 13
574080 6.1
624000 3.9
673920 3.7
723840 3
773760 1.1
823680 0.3
873600 2.5
923520 9
973440 17.3
1023360 25.5
1073280 30.5
1123200 32
1173120 32.3
1223040 34.7
1272960 41
1322880 50.1
1372800 57.9
1422720 61.4
1472640 63.1
1522560 64.9
1572480 69.9
1622400 78.4
1672320 88
1722240 95.3
1772160 98.7
1822080 99.6
1872000 99.6
1921920 99.6
1971840 99.6
2021760 99.6
2071680 99.5
2121600 99.4
2171520 99.5
2221440 99.7
2271360 99.8
2321280 99.8
2371200 99.8
2421120 99.8
2471040 99.8
2520960 99.8
2570880 99.9
2620800 100
2670720 99.9
2720640 99.8
2770560 99.7
2820480 98.5
2870400 90.5
2920320 81.7
2970240 75.6
3020160 68.4
3070080 62.4
3120000 57.8
3169920 53.7
3219840 46.3
3269760 38
3319680 33
3369600 31.6
3419520 32
3469440 28.2
3519360 25.4
3569280 21.4
3619200 16
3669120 10.2
3719040 7.7
3768960 6.1
3818880 2.3
3868800 1.7
3918720 0.1
3968640 0
4018560 0
4068480 0
4118400 0
4168320 0
4218240 0
4268160 0
4318080 0
4368000 0
4417920 0.1
4467840 0.1
4517760 0.1
4567680 0.1
4617600 0.1
4667520 0.1
4717440 0.1
4767360 0.1
4817280 0.1
4867200 0.1
4917120 0
4967040 0
5016960 0
5066880 0
5116800 0
5166720 0
5216640 0
5266560 0
5316480 0
5366400 0
5416320 0
5466240 0
5516160 0
5566080 0
5616000 0
5665920 0
5715840 0
5765760 0
5815680 0
5865600 0
5915520 0
5965440 0
6015360 0
6065280 0
6115200 0
6165120 0
6215040 0
6264960 0
6314880 0
6364800 0
6414720 0
6464640 0
6514560 0
6564480 0
6614400 0
6664320 0
6714240 0
6764160 0
6814080 0
};
\addlegendentry{\scriptsize{Ran Out Of Time}}
\addplot [very thick, color3]
table {%
49920 0
74880 0
99840 0
124800 0
149760 0
174720 0
199680 0
224640 0
249600 0
274560 0
324480 0
374400 0
424320 0
474240 0
524160 0
574080 0
624000 0
673920 0
723840 0
773760 0
823680 0
873600 0
923520 0
973440 0
1023360 0
1073280 0
1123200 0
1173120 0
1223040 0
1272960 0
1322880 0
1372800 0
1422720 0
1472640 0
1522560 0
1572480 0
1622400 0
1672320 0
1722240 0
1772160 0
1822080 0
1872000 0
1921920 0
1971840 0
2021760 0
2071680 0
2121600 0
2171520 0
2221440 0
2271360 0
2321280 0
2371200 0
2421120 0
2471040 0
2520960 0
2570880 0
2620800 0
2670720 0
2720640 0
2770560 0.1
2820480 1.2
2870400 9.1
2920320 17.9
2970240 24
3020160 31.1
3070080 37
3120000 41.4
3169920 45.5
3219840 53
3269760 61.2
3319680 66.3
3369600 67.8
3419520 67.4
3469440 71.2
3519360 74.1
3569280 78.2
3619200 83.8
3669120 89.7
3719040 92.2
3768960 93.9
3818880 97.7
3868800 98.3
3918720 99.9
3968640 100
4018560 100
4068480 100
4118400 100
4168320 100
4218240 100
4268160 100
4318080 100
4368000 100
4417920 99.9
4467840 99.9
4517760 99.9
4567680 99.9
4617600 99.9
4667520 99.8
4717440 99.8
4767360 99.8
4817280 99.8
4867200 99.8
4917120 99.9
4967040 99.9
5016960 99.9
5066880 99.9
5116800 99.9
5166720 100
5216640 100
5266560 100
5316480 100
5366400 100
5416320 100
5466240 100
5516160 100
5566080 100
5616000 100
5665920 100
5715840 100
5765760 100
5815680 100
5865600 100
5915520 100
5965440 100
6015360 100
6065280 100
6115200 100
6165120 100
6215040 99.9
6264960 99.9
6314880 99.9
6364800 99.9
6414720 99.9
6464640 99.9
6514560 99.8
6564480 99.8
6614400 99.8
6664320 99.8
6714240 99.9
6764160 99.9
6814080 99.9
};
\addlegendentry{\scriptsize{Reached Goal}}
\addlegendimage{/pgfplots/refstyle=plot1}\addlegendentry{\scriptsize{Discounted Return}}
\end{axis}

\end{tikzpicture}


==> IROS2021 - ArXiv - Cooperative Assistance/plots/learning_curve_tikz.tex <==
\begin{figure}[tb]
       % \centering
       \parbox{\columnwidth}{
       % \vspace{2mm}
         \vspace{1.5mm}
         \begin{tikzpicture}%[trim left=0]
                \begin{axis}[
                        axis x line=bottom,
                        axis y line=middle,
                        % xtick pos=both,
                        % xtick style={color=black},
                        axis line style={-},
                        %x label style={at={(axis description cs:0.5,0.05)},anchor=north},
                        x label style={at={(axis description cs:0.5,-0.15)},anchor=north},
                        y label style={at={(axis description cs:-0.1,0.5)},rotate=90,anchor=south},
                        xlabel={\small Total Environment Steps},
                        ylabel={\small Discounted Return},
                        ytick distance={5},
                        enlarge y limits=true,
                        width=0.95\columnwidth,
                        height=0.5\columnwidth,
                        grid = major,
                        grid style={dashed, gray!30},
                        legend style={at={(0.02,1)}, anchor=north west},
                        yticklabel style = {font=\scriptsize,xshift=0.5ex},
                        xticklabel style = {font=\scriptsize,yshift=0.5ex},
                        every x tick scale label/.style={at={(1,-0.1)},xshift=1pt,anchor=north,inner sep=0pt}
                     ]
                    \draw (axis description cs:0,1) -- (axis description cs:1,1);
                    \addplot[smooth, no markers, black, thick] table[x=steps,y=return,col sep=comma] {plots/data.csv};
                    \label{return_plot}
                \end{axis}

                \begin{axis}[
                        axis x line=bottom,
                        axis y line=right,
                        axis line style={-},
                        x label style={opacity=0},
                        y label style={at={(axis description cs:1.14,0.5)},rotate=0,anchor=south},
                        xlabel={},
                        ytick distance={25},
                        ylabel={\small Outcome [\%]},
                        enlarge y limits=true,
                        width=0.95\columnwidth, 
                        height=0.5\columnwidth,
                        legend style={fill opacity=1, draw opacity=1, text opacity=1, at={(1,0.15)}, anchor=south east, nodes={scale=0.8, transform shape}, draw=none},
                        yticklabel style = {font=\scriptsize,xshift=-0.5ex},
                        xticklabel style = {opacity=0},
                     ]
                    \addplot[smooth, no markers, OliveGreen, thick, dash dot] table[x=steps,y=won,col sep=comma] {plots/data.csv};
                    \addlegendentry{\small{Reached Goal}}
                    \addplot[smooth, no markers, red, thick, dashed] table[x=steps,y=lost,col sep=comma] {plots/data.csv};
                    \addlegendentry{\small{Lost Grasp}}
                    \addplot[smooth, no markers, blue, thick, dotted] table[x=steps,y=time,col sep=comma] {plots/data.csv};
                    \addlegendentry{\small{Ran Out of Time}}
                    \addlegendimage{/pgfplots/refstyle=return_plot}\addlegendentry{\small{Discounted Return}}
                    \begin{scope}[on background layer]
                        \fill[red,opacity=0.1] ({rel axis cs:0,0}) rectangle ({rel axis cs:0.2,1});
                        \fill[blue,opacity=0.1] ({rel axis cs:0.2,0}) rectangle ({rel axis cs:0.46,1});
                        \fill[OliveGreen,opacity=0.1] ({rel axis cs:0.46,0}) rectangle ({rel axis cs:1,1});
                    \end{scope}
                \end{axis}
                % \begin{axis}[
                % thick,
                % smooth,
                % no markers,
                % width=0.95\columnwidth, 
                % height=0.5\columnwidth,
                % ]
                %     \addplot+[name path=A,black, opacity=0.8] {0};
                %     \addplot+[name path=B,black, opacity=0.8] {-10};

                %     \addplot[blue!50] fill between[of=A and B];
                % \end{axis}
            \end{tikzpicture}
       }
       \vspace{-0.2cm}
       \caption{Smoothed learning curve for one example training run. Discounted return and percentage of the three different outcomes are shown over steps in the learning environment.}
       \label{fig:learning_curve}
       \vspace{-0.5cm}
\end{figure}


==> IROS2021 - ArXiv - Cooperative Assistance/results_table.tex <==
    \begin{table*}
      \centering
        \vspace{1.5mm}
      \caption{Evaluation results for human and hybrid teams. Metrics from Section~\ref{sec:methods:metrics} are averaged over ten trials (n~=~10). The teams are abbreviated as illustrated in Fig.~\ref{fig:teams}. Simulation steps with collisions are observed between gripper and liver (Col-GL), cauter and liver (Col-CL), cauter and gallbladder (Col-CG), and between instruments (Col-II).}
      \begin{tabular*}{\textwidth}{ @{\extracolsep{\fill}} lrrrrrrrrr}
        \toprule
        Metric         & HuT1            & HuT2           & HuT3            & HyT1           & HyT2          & HyT3          & HyT4          & HyT5           & HyT6          \\
        \midrule
        Success [\%]   & $100 \pm 0$     & $100 \pm 0$    & $100 \pm 0$     & $100 \pm 0$    & $100 \pm 0$   & $100 \pm 0$   & $100 \pm 0$   & $100 \pm 0$    & $100 \pm 0$   \\
        Time [s]       & $19.8 \pm 2.6$  & $14.2 \pm 4.6$ & $13.2 \pm 3.3$  & $10.1 \pm 2.3$ & $5.7 \pm 0.4$ & $7.9 \pm 0.6$ & $5.7 \pm 0.3$ & $7.3 \pm 0.9$  & $5.1 \pm 0.4$ \\
        PL-G [mm]      & $295 \pm 12$    & $302 \pm 9$    & $315 \pm 24$    & $298 \pm 12$   & $257 \pm 5$   & $296 \pm 10$  & $266 \pm 9$   & $300 \pm 13$   & $261 \pm 8$   \\
        PL-C [mm]      & $297 \pm 46$    & $344 \pm 29$   & $341 \pm 56$    & $284 \pm 37$   & $347 \pm 29$  & $269 \pm 26$  & $359 \pm 14$  & $247\pm 37$    & $300 \pm 29$  \\
        Col-GL [steps] & $2.4 \pm 7.2$   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$   & $0.0 \pm 0.0$  & $0.2 \pm 0.4$ & $0.1 \pm 0.3$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.3 \pm 0.9$ \\
        Col-CL [steps] & $13.7 \pm 41.1$ & $3.4 \pm 10.2$ & $0.0 \pm 0.0$   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $7.8 \pm 23.4$ & $0.0 \pm 0.0$ \\
        Col-CG [steps] & $3.7 \pm 11.1$  & $1.5 \pm 4.2$  & $14.1 \pm 15.8$ & $1.1 \pm 3.3$  & $0.2 \pm 0.4$ & $1.7 \pm 4.0$ & $0.1 \pm 0.3$ & $0.0 \pm 0.0$  & $1.8 \pm 3.1$ \\
        Col-II [steps] & $0.0 \pm 0.0$   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$   & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        \bottomrule
      \end{tabular*}
      \label{tab:human_hybrid_team}
      \vspace{-0.5cm}
    \end{table*}


==> IROS2021 - ArXiv - Cooperative Assistance/results_table_human.tex <==
    \begin{table}
      \centering
      \caption{Evaluation results for the human teams. The metrics from \ref{sec:methods:metrics} are calculated as a mean over ten trials (n=10). The teams are abbreviated as illustrated in Fig.~\ref{fig:teams}. Simulation steps with collisions were observed between gripper and liver (Col-GL), cauter and liver (Col-CL), cauter and gallbladder (Col-CG), and between instruments (Col-II).}
      \begin{tabular*}{\columnwidth}{ @{\extracolsep{\fill}} lrrr}
        \toprule
        Metric         & HuT1            & HuT2            & HuT3           \\
        \midrule
        Success [\%]   & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      \\
        DR             & $8.47 \pm xx$    & $17.33 \pm xx$   & $11.90 \pm xx$   \\
        Time [s]       & $19.84 \pm 2.60$ & $14.23 \pm 4.57$ & $13.17 \pm 3.25$ \\
        PL-G [mm]      & $294.7 \pm 11.6$ & $301.7 \pm 9.0$  & $315.1 \pm 24.3$ \\
        PL-C [mm]      & $296.6 \pm 45.7$ & $343.9 \pm 28.9$ & $340.7 \pm 56.0$ \\
        Col-GL [steps] & $2.4 \pm 7.2$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    \\
        Col-CL [steps] & $13.7 \pm 41.1$  & $3.4 \pm 10.2$   & $0.0 \pm 0.0$    \\
        Col-CG [steps] & $3.7 \pm 11.1$   & $1.5 \pm 4.2$    & $14.1 \pm 15.8$  \\
        Col-II [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    \\
        \bottomrule
      \end{tabular*}
      \label{tab:human_team}
      \vspace{-0.2cm}
    \end{table}


==> IROS2021 - ArXiv - Cooperative Assistance/results_table_hybrid.tex <==
    \begin{table*}
      \centering
      \caption{Evaluation results for the hybrid teams. The abbreviations follow the same convention as TABLE~\ref{tab:human_team}.}
      \begin{tabular*}{\textwidth}{ @{\extracolsep{\fill}} lrrrrrr}
        \toprule
        Metric         & HyT1            & HyT2            & HyT3            & HyT4            & HyT5            & HyT6 \\
        \midrule
        Success [\%]   & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$   \\
        DR             & x     & x       & x     & x       & x     & x     \\
        Time [s]       & $10.14 \pm 2.28$ & $5.69 \pm 0.43$  & $7.93 \pm 0.65$  & $5.71 \pm 0.30$  & $7.33 \pm 0.93$  & $5.08 \pm 0.36$  \\
        PL-G [mm]      & $298.5 \pm 11.6$ & $256.8 \pm 5.2$  & $295.8 \pm 10.3$ & $265.5 \pm 8.8$  & $299.7 \pm 12.9$ & $261.0 \pm 7.9$ \\
        PL-C [mm]      & $284.1 \pm 36.8$ & $347.5 \pm 28.9$ & $268.5 \pm 26.5$ & $358.5 \pm 14.5$ & $247.0 \pm 36.9$ & $300.1 \pm 29.2$ \\
        Col-GL [steps] & $0.0 \pm 0.0$    & $0.2 \pm 0.4$    & $0.1 \pm 0.3$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$   & $0.3 \pm 0.9$   \\
        Col-CL [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $7.8 \pm 23.4$   & $0.0 \pm 0.0$   \\
        Col-CG [steps] & $1.1 \pm 3.3$    & $0.2 \pm 0.4$    & $1.7 \pm 4.0$    & $0.1 \pm 0.3$    & $0.0 \pm 0.0$   & $1.8 \pm 3.1$   \\
        Col-II [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$   & $0.0 \pm 0.0$   \\
        \bottomrule
      \end{tabular*}
      \label{tab:hybrid_team}
      \vspace{-0.2cm}
    \end{table*}


==> plots/learning_curve.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.266666666666667,0.466666666666667,0.666666666666667}
\definecolor{color1}{rgb}{0.933333333333333,0.4,0.466666666666667}
\definecolor{color2}{rgb}{0.133333333333333,0.533333333333333,0.2}
\definecolor{color3}{rgb}{0.8,0.733333333333333,0.266666666666667}

\begin{axis}[
x grid style={white!69.0196078431373!black},
xlabel={\scriptsize Total Environment Steps},
xmin=-288288, xmax=7152288,
xtick pos=both,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={\scriptsize Discounted Return},
ymin=-22.1813958573089, ymax=-7.27974484059465,
ytick pos=left,
ytick style={color=black}
]
\addplot [very thick, color0]
table {%
49920 -21.5040480838219
74880 -21.1827974647543
99840 -20.7382724465402
124800 -20.4181807455722
149760 -20.1672456540431
174720 -20.0306862873427
199680 -20.108840957863
224640 -20.0768693775711
249600 -20.0378520216418
274560 -20.0484475850687
324480 -19.8513096398831
374400 -19.702423021939
424320 -19.617712030216
474240 -19.5958992299732
524160 -19.5588585185347
574080 -19.5899820385266
624000 -19.4616895139411
673920 -19.3399181157626
723840 -19.2805551285742
773760 -19.1953316922821
823680 -19.1330114576469
873600 -19.1003669646225
923520 -19.0770256191707
973440 -18.9917650777353
1023360 -18.9892890571493
1073280 -18.9419460988782
1123200 -18.8416428681302
1173120 -18.7880762867179
1223040 -18.6650964808592
1272960 -18.3926056123042
1322880 -17.969604018927
1372800 -17.4307253986179
1422720 -16.9022332596665
1472640 -16.4140599940098
1522560 -15.9027247871292
1572480 -15.3560557761683
1622400 -14.8832678631575
1672320 -14.4070487135294
1722240 -13.9299480521507
1772160 -13.5643457671856
1822080 -13.3919921497161
1872000 -13.491008567069
1921920 -13.6495731080686
1971840 -13.6608632360486
2021760 -13.6251105166927
2071680 -13.5907730054541
2121600 -13.5631835746639
2171520 -13.5565636511123
2221440 -13.5604444871481
2271360 -13.5584916698884
2321280 -13.567112531402
2371200 -13.4477978259416
2421120 -13.2271443184031
2471040 -13.0863694027688
2520960 -13.0067422858907
2570880 -12.9995341474053
2620800 -13.1005547885826
2670720 -13.2478727952339
2720640 -13.4528035787561
2770560 -13.6331957449306
2820480 -13.5828257540864
2870400 -13.3001354649258
2920320 -13.0451509928973
2970240 -12.848182217605
3020160 -12.5773408160109
3070080 -12.2527934928604
3120000 -11.8524058616213
3169920 -11.4460235276974
3219840 -10.9103904471533
3269760 -10.3758936058991
3319680 -10.1493774685482
3369600 -10.0611940761428
3419520 -10.2197463160194
3469440 -10.1352382335704
3519360 -10.1267905929482
3569280 -10.0011823692447
3619200 -9.88124232622069
3669120 -9.64674547547582
3719040 -9.5245430163311
3768960 -9.43407828971426
3818880 -9.27540347530714
3868800 -9.10150903485422
3918720 -8.71699690554348
3968640 -8.58279913649857
4018560 -8.51728603798155
4068480 -8.48575773869541
4118400 -8.39866930883652
4168320 -8.39731709804498
4218240 -8.36287584317581
4268160 -8.35503501809728
4318080 -8.2807509426549
4368000 -8.30833266943386
4417920 -8.32450831899301
4467840 -8.33281282756494
4517760 -8.23518912028296
4567680 -8.19406078473346
4617600 -8.19622377358428
4667520 -8.17646914452722
4717440 -8.15214283190572
4767360 -8.12502481377371
4817280 -8.14960576665908
4867200 -8.14080271033512
4917120 -8.16441442520513
4967040 -8.14264039263577
5016960 -8.14074911589156
5066880 -8.13263549562361
5116800 -8.12330619505144
5166720 -8.11831066092713
5216640 -8.11549596177326
5266560 -8.09403924244443
5316480 -8.08351237392855
5366400 -8.05991360155514
5416320 -8.00142823627823
5466240 -8.01630599061512
5516160 -8.01839797688231
5566080 -8.01551814234745
5616000 -7.99695626918515
5665920 -8.01534030314152
5715840 -8.00138148613027
5765760 -7.99625540525388
5815680 -7.98587233202064
5865600 -8.01583181973664
5915520 -8.04199977527534
5965440 -8.04095356090127
6015360 -8.05091459449297
6065280 -8.0429501848792
6115200 -8.05614699202149
6165120 -8.0502487393353
6215040 -8.05222055260378
6264960 -8.07653399641677
6314880 -8.07916527726033
6364800 -8.04066320719996
6414720 -8.0273415804971
6464640 -8.05116276585494
6514560 -8.03536637890315
6564480 -8.03292787783407
6614400 -8.00431567053931
6664320 -7.97955364769339
6714240 -7.99436547182909
6764160 -7.97718630405352
6814080 -7.95709261408166
};
\label{plot1}
\end{axis}

\begin{axis}[
axis y line=right,
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, at={(0.91,0.5)}, anchor=east, draw=none},
x grid style={white!69.0196078431373!black},
xmin=-288288, xmax=7152288,
xtick pos=both,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Outcome (\%)},
ymin=0, ymax=105,
ytick pos=right,
ytick style={color=black},
yticklabel style={anchor=west}
]
\addplot [very thick, color1]
table {%
49920 0
74880 18.5
99840 43.6666666666667
124800 50.5
149760 46.4
174720 43.8333333333333
199680 48.7142857142857
224640 54.875
249600 59
274560 61
324480 70.2
374400 76.5
424320 77.1
474240 80
524160 87
574080 93.9
624000 96.1
673920 96.3
723840 97
773760 98.9
823680 99.7
873600 97.5
923520 91
973440 82.7
1023360 74.5
1073280 69.5
1123200 68
1173120 67.7
1223040 65.3
1272960 59
1322880 49.9
1372800 42.1
1422720 38.6
1472640 36.9
1522560 35.1
1572480 30.1
1622400 21.6
1672320 12
1722240 4.7
1772160 1.3
1822080 0.4
1872000 0.4
1921920 0.4
1971840 0.4
2021760 0.4
2071680 0.5
2121600 0.6
2171520 0.5
2221440 0.3
2271360 0.2
2321280 0.2
2371200 0.2
2421120 0.2
2471040 0.2
2520960 0.2
2570880 0.1
2620800 0
2670720 0.1
2720640 0.2
2770560 0.2
2820480 0.3
2870400 0.4
2920320 0.4
2970240 0.4
3020160 0.5
3070080 0.6
3120000 0.8
3169920 0.8
3219840 0.7
3269760 0.8
3319680 0.7
3369600 0.6
3419520 0.6
3469440 0.6
3519360 0.5
3569280 0.4
3619200 0.2
3669120 0.1
3719040 0.1
3768960 0
3818880 0
3868800 0
3918720 0
3968640 0
4018560 0
4068480 0
4118400 0
4168320 0
4218240 0
4268160 0
4318080 0
4368000 0
4417920 0
4467840 0
4517760 0
4567680 0
4617600 0
4667520 0.1
4717440 0.1
4767360 0.1
4817280 0.1
4867200 0.1
4917120 0.1
4967040 0.1
5016960 0.1
5066880 0.1
5116800 0.1
5166720 0
5216640 0
5266560 0
5316480 0
5366400 0
5416320 0
5466240 0
5516160 0
5566080 0
5616000 0
5665920 0
5715840 0
5765760 0
5815680 0
5865600 0
5915520 0
5965440 0
6015360 0
6065280 0
6115200 0
6165120 0
6215040 0.1
6264960 0.1
6314880 0.1
6364800 0.1
6414720 0.1
6464640 0.1
6514560 0.2
6564480 0.2
6614400 0.2
6664320 0.2
6714240 0.1
6764160 0.1
6814080 0.1
};
\addlegendentry{\scriptsize{Lost Grasp}}
\addplot [very thick, color2]
table {%
49920 100
74880 81.5
99840 56.3333333333333
124800 49.5
149760 53.6
174720 56.1666666666667
199680 51.2857142857143
224640 45.125
249600 41
274560 39
324480 29.8
374400 23.5
424320 22.9
474240 20
524160 13
574080 6.1
624000 3.9
673920 3.7
723840 3
773760 1.1
823680 0.3
873600 2.5
923520 9
973440 17.3
1023360 25.5
1073280 30.5
1123200 32
1173120 32.3
1223040 34.7
1272960 41
1322880 50.1
1372800 57.9
1422720 61.4
1472640 63.1
1522560 64.9
1572480 69.9
1622400 78.4
1672320 88
1722240 95.3
1772160 98.7
1822080 99.6
1872000 99.6
1921920 99.6
1971840 99.6
2021760 99.6
2071680 99.5
2121600 99.4
2171520 99.5
2221440 99.7
2271360 99.8
2321280 99.8
2371200 99.8
2421120 99.8
2471040 99.8
2520960 99.8
2570880 99.9
2620800 100
2670720 99.9
2720640 99.8
2770560 99.7
2820480 98.5
2870400 90.5
2920320 81.7
2970240 75.6
3020160 68.4
3070080 62.4
3120000 57.8
3169920 53.7
3219840 46.3
3269760 38
3319680 33
3369600 31.6
3419520 32
3469440 28.2
3519360 25.4
3569280 21.4
3619200 16
3669120 10.2
3719040 7.7
3768960 6.1
3818880 2.3
3868800 1.7
3918720 0.1
3968640 0
4018560 0
4068480 0
4118400 0
4168320 0
4218240 0
4268160 0
4318080 0
4368000 0
4417920 0.1
4467840 0.1
4517760 0.1
4567680 0.1
4617600 0.1
4667520 0.1
4717440 0.1
4767360 0.1
4817280 0.1
4867200 0.1
4917120 0
4967040 0
5016960 0
5066880 0
5116800 0
5166720 0
5216640 0
5266560 0
5316480 0
5366400 0
5416320 0
5466240 0
5516160 0
5566080 0
5616000 0
5665920 0
5715840 0
5765760 0
5815680 0
5865600 0
5915520 0
5965440 0
6015360 0
6065280 0
6115200 0
6165120 0
6215040 0
6264960 0
6314880 0
6364800 0
6414720 0
6464640 0
6514560 0
6564480 0
6614400 0
6664320 0
6714240 0
6764160 0
6814080 0
};
\addlegendentry{\scriptsize{Ran Out Of Time}}
\addplot [very thick, color3]
table {%
49920 0
74880 0
99840 0
124800 0
149760 0
174720 0
199680 0
224640 0
249600 0
274560 0
324480 0
374400 0
424320 0
474240 0
524160 0
574080 0
624000 0
673920 0
723840 0
773760 0
823680 0
873600 0
923520 0
973440 0
1023360 0
1073280 0
1123200 0
1173120 0
1223040 0
1272960 0
1322880 0
1372800 0
1422720 0
1472640 0
1522560 0
1572480 0
1622400 0
1672320 0
1722240 0
1772160 0
1822080 0
1872000 0
1921920 0
1971840 0
2021760 0
2071680 0
2121600 0
2171520 0
2221440 0
2271360 0
2321280 0
2371200 0
2421120 0
2471040 0
2520960 0
2570880 0
2620800 0
2670720 0
2720640 0
2770560 0.1
2820480 1.2
2870400 9.1
2920320 17.9
2970240 24
3020160 31.1
3070080 37
3120000 41.4
3169920 45.5
3219840 53
3269760 61.2
3319680 66.3
3369600 67.8
3419520 67.4
3469440 71.2
3519360 74.1
3569280 78.2
3619200 83.8
3669120 89.7
3719040 92.2
3768960 93.9
3818880 97.7
3868800 98.3
3918720 99.9
3968640 100
4018560 100
4068480 100
4118400 100
4168320 100
4218240 100
4268160 100
4318080 100
4368000 100
4417920 99.9
4467840 99.9
4517760 99.9
4567680 99.9
4617600 99.9
4667520 99.8
4717440 99.8
4767360 99.8
4817280 99.8
4867200 99.8
4917120 99.9
4967040 99.9
5016960 99.9
5066880 99.9
5116800 99.9
5166720 100
5216640 100
5266560 100
5316480 100
5366400 100
5416320 100
5466240 100
5516160 100
5566080 100
5616000 100
5665920 100
5715840 100
5765760 100
5815680 100
5865600 100
5915520 100
5965440 100
6015360 100
6065280 100
6115200 100
6165120 100
6215040 99.9
6264960 99.9
6314880 99.9
6364800 99.9
6414720 99.9
6464640 99.9
6514560 99.8
6564480 99.8
6614400 99.8
6664320 99.8
6714240 99.9
6764160 99.9
6814080 99.9
};
\addlegendentry{\scriptsize{Reached Goal}}
\addlegendimage{/pgfplots/refstyle=plot1}\addlegendentry{\scriptsize{Discounted Return}}
\end{axis}

\end{tikzpicture}


==> results_table_human.tex <==
    \begin{table}
      \centering
      \caption{Evaluation results for the human teams. The metrics from \ref{sec:methods:metrics} are calculated as a mean over ten trials (n=10). The teams are abbreviated as illustrated in Fig.~\ref{fig:teams}. Simulation steps with collisions were observed between gripper and liver (Col-GL), cauter and liver (Col-CL), cauter and gallbladder (Col-CG), and between instruments (Col-II).}
      \begin{tabular*}{\columnwidth}{ @{\extracolsep{\fill}} lrrr}
        \toprule
        Metric         & HuT1            & HuT2            & HuT3           \\
        \midrule
        Success [\%]   & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      \\
        DR             & $8.47 \pm xx$    & $17.33 \pm xx$   & $11.90 \pm xx$   \\
        Time [s]       & $19.84 \pm 2.60$ & $14.23 \pm 4.57$ & $13.17 \pm 3.25$ \\
        PL-G [mm]      & $294.7 \pm 11.6$ & $301.7 \pm 9.0$  & $315.1 \pm 24.3$ \\
        PL-C [mm]      & $296.6 \pm 45.7$ & $343.9 \pm 28.9$ & $340.7 \pm 56.0$ \\
        Col-GL [steps] & $2.4 \pm 7.2$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    \\
        Col-CL [steps] & $13.7 \pm 41.1$  & $3.4 \pm 10.2$   & $0.0 \pm 0.0$    \\
        Col-CG [steps] & $3.7 \pm 11.1$   & $1.5 \pm 4.2$    & $14.1 \pm 15.8$  \\
        Col-II [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    \\
        \bottomrule
      \end{tabular*}
      \label{tab:human_team}
      \vspace{-0.2cm}
    \end{table}


==> results_table_hybrid.tex <==
    \begin{table*}
      \centering
      \caption{Evaluation results for the hybrid teams. The abbreviations follow the same convention as TABLE~\ref{tab:human_team}.}
      \begin{tabular*}{\textwidth}{ @{\extracolsep{\fill}} lrrrrrr}
        \toprule
        Metric         & HyT1            & HyT2            & HyT3            & HyT4            & HyT5            & HyT6 \\
        \midrule
        Success [\%]   & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$      & $100 \pm 0$   \\
        DR             & x     & x       & x     & x       & x     & x     \\
        Time [s]       & $10.14 \pm 2.28$ & $5.69 \pm 0.43$  & $7.93 \pm 0.65$  & $5.71 \pm 0.30$  & $7.33 \pm 0.93$  & $5.08 \pm 0.36$  \\
        PL-G [mm]      & $298.5 \pm 11.6$ & $256.8 \pm 5.2$  & $295.8 \pm 10.3$ & $265.5 \pm 8.8$  & $299.7 \pm 12.9$ & $261.0 \pm 7.9$ \\
        PL-C [mm]      & $284.1 \pm 36.8$ & $347.5 \pm 28.9$ & $268.5 \pm 26.5$ & $358.5 \pm 14.5$ & $247.0 \pm 36.9$ & $300.1 \pm 29.2$ \\
        Col-GL [steps] & $0.0 \pm 0.0$    & $0.2 \pm 0.4$    & $0.1 \pm 0.3$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$   & $0.3 \pm 0.9$   \\
        Col-CL [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $7.8 \pm 23.4$   & $0.0 \pm 0.0$   \\
        Col-CG [steps] & $1.1 \pm 3.3$    & $0.2 \pm 0.4$    & $1.7 \pm 4.0$    & $0.1 \pm 0.3$    & $0.0 \pm 0.0$   & $1.8 \pm 3.1$   \\
        Col-II [steps] & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$    & $0.0 \pm 0.0$   & $0.0 \pm 0.0$   \\
        \bottomrule
      \end{tabular*}
      \label{tab:hybrid_team}
      \vspace{-0.2cm}
    \end{table*}

